Beyond Dark Knowledge: Mixup-Based Distillation for Reliable Predictions

Knowledge Distillation (KD) and mixup have proven effective at inducing smoothness in class boundaries; KD captures inherent class relationships in probability distributions, and mixup enforces them through convex combinations of inputs. Their interaction, however, remains poorly understood, particularly when mixup is applied only during student training. In this setting, the teacher is queried on inputs drawn from a vicinal distribution it never saw during training, a controlled mismatch whose effect on knowledge transfer has not been characterised. We show that this mismatch causes the teacher's supervisory signal to be dominated by distributional confusion rather than inter-class structure. Despite it, the student does not merely imitate the teacher: it independently acquires greater linearity in the vicinal region, a structural property that the teacher lacks, and goes beyond dark-knowledge transfer. KD with mixup consistently improves student accuracy and reduces overconfidence by an order of magnitude relative to the baseline, across CIFAR and ImageNet with varying-capacity teachers. Crucially, calibration propagates from teacher to student independently of accuracy transfer, and temperature scaling governs a measurable accuracy-calibration trade-off that becomes more pronounced under vicinal training. These results reframe mixup distillation not as a degraded version of standard KD, but as a richer transfer channel that simultaneously shapes discriminative performance, uncertainty estimation, and representational geometry.

==> calibration.tex <==
We therefore ask a question—can a calibrated student be distilled from an uncalibrated teacher?,
Calibration is a quantification of uncertainty. Uncertainty can be broadly divided into two types: data uncertainty and model uncertainty.
model uncertainty can be minimised by adjusting the confidence of the model.
Data unsertanty no se puede cuando se trabaja con pretrained models y transfer knowledge and fine tuning.
The goal is to reduce data uncertanty
Here, n represents the number of samples in the dataset. When the teacher is uncalibrated, and the temperature parameter (τ ) is in close proximity to 1, the loss function LKD compels the student to mimic the distribution of the uncalibrated teacher.
Consequently, the student also becomes uncalibrated.

if Temperature is xtreamly increased it can affect the knowledge transfer. Finding a optimal T is critical for enhancing calibration. Even when the classification loss is reduced to zero, the CE loss may persist, leading the optimizer to continue inimizing it. This persistence in optimization can impact the calibration of the model, potentially causing deviations from the desired calibration state.
MixUP interpolation regularizes the decision boundaries of the model, reducing overconfidence
and improving calibration.
Mixup is also shown to reduce the overconfidence
error of the model.

==> images/loss_by_temperature.tex <==
%% Creator: Inkscape 1.3.2 (091e20e, 2023-11-25, custom), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'loss_by_temperature.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{680.2020874bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.61577074)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{loss_by_temperature.pdf}}%
    \put(0.18773173,0.00767539){\color[rgb]{0.33333333,0.33333333,0.33333333}\makebox(0,0)[lt]{\lineheight{0.30000001}\smash{\begin{tabular}[t]{l}T=2\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{loss_by_temperature.pdf}}%
    \put(0.39839277,0.00767539){\color[rgb]{0.33333333,0.33333333,0.33333333}\makebox(0,0)[lt]{\lineheight{0.30000001}\smash{\begin{tabular}[t]{l}T=4\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{loss_by_temperature.pdf}}%
    \put(0.60943764,0.00767539){\color[rgb]{0.33333333,0.33333333,0.33333333}\makebox(0,0)[lt]{\lineheight{0.30000001}\smash{\begin{tabular}[t]{l}T=6\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{loss_by_temperature.pdf}}%
    \put(0.78276745,0.00720053){\color[rgb]{0.33333333,0.33333333,0.33333333}\makebox(0,0)[lt]{\lineheight{0.30000001}\smash{\begin{tabular}[t]{l}T=$\sigma$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{loss_by_temperature.pdf}}%
  \end{picture}%
\endgroup%


==> teacherReliability.tex <==
\section{Teacher Reliability Under Mixup}

The formulation presented in the previous section highlights a fundamental property of distillation under Mixup: the teacher network is queried on inputs that lie outside the distribution on which it was originally trained. In this section we analyze how this distributional shift affects the reliability and calibration of teacher predictions.

\subsection{Vicinal Distribution and Interpolation Regime}

Mixup training generates samples from a vicinal distribution $\nu_{mixup}$ defined over convex combinations of training examples. This formulation can be interpreted within the Vicinal Risk Minimization (VRM) framework introduced by Vapnik, where the empirical data distribution is replaced by a local neighborhood around each training sample \cite{chapelle2000vicinal}. 

Under VRM, the learning objective approximates the expected risk

\begin{equation}
R(f) = \mathbb{E}_{(x,y)\sim P_{data}}
\left[
\ell(f(x),y)
\right]
\end{equation}

by minimizing the vicinal risk

\begin{equation}
R_{vic}(f) =
\mathbb{E}_{(\tilde{x},\tilde{y})\sim\nu_{mixup}}
\left[
\ell(f(\tilde{x}),\tilde{y})
\right].
\end{equation}

This formulation encourages the model to behave smoothly in regions between training examples, effectively enforcing a linear behavior between samples \cite{zhang2017mixup}. 

However, in the distillation setting considered in this work, the teacher network is not optimized with respect to the vicinal distribution. Consequently, when queried with interpolated inputs

\begin{equation}
\tilde{x} = \lambda x_i + (1-\lambda)x_j
\end{equation}

the teacher operates in a regime that may not correspond to the regions of highest training density.


\subsection{Prediction Uncertainty on Interpolated Samples}

Let $p_t(x)$ denote the teacher predictive distribution. The uncertainty of the prediction can be measured through the entropy of the output distribution

\begin{equation}
H(p_t(x)) =
- \sum_{k=1}^{K} p_t(x)_k \log p_t(x)_k .
\end{equation}

We analyze the expected entropy under the two input distributions:

\begin{equation}
\mathcal{H}_{data} =
\mathbb{E}_{x\sim P_{data}}
\left[
H(p_t(x))
\right]
\end{equation}

\begin{equation}
\mathcal{H}_{mixup} =
\mathbb{E}_{\tilde{x}\sim\nu_{mixup}}
\left[
H(p_t(\tilde{x}))
\right].
\end{equation}

The difference

\begin{equation}
\Delta H =
\mathcal{H}_{mixup} - \mathcal{H}_{data}
\end{equation}

characterizes how the predictive uncertainty of the teacher changes when evaluated on interpolated inputs.

If Mixup samples lie near decision boundaries, the teacher is expected to produce higher entropy predictions due to ambiguity between classes. Conversely, if the teacher extrapolates confidently outside the training manifold, predictions may become overconfident.


\subsection{Confidence Calibration Under Distribution Shift}

Beyond entropy, the reliability of the teacher can be analyzed through calibration. Calibration measures the alignment between predicted confidence and empirical accuracy.

Let

\begin{equation}
conf(x) = \max_k p_t(x)_k
\end{equation}

denote the confidence of the prediction. A well calibrated model satisfies

\begin{equation}
\mathbb{P}(\hat{y}=y \mid conf(x)=c) = c .
\end{equation}

In practice calibration is estimated using the Expected Calibration Error (ECE)

\begin{equation}
ECE =
\sum_{m=1}^{M}
\frac{|B_m|}{N}
\left|
acc(B_m) - conf(B_m)
\right|.
\end{equation}

Modern deep networks are often overconfident, producing confidence estimates that exceed their empirical accuracy \cite{mishra2025beyond}. 

Data augmentation strategies such as Mixup have been shown to regularize model predictions and improve calibration by reducing extreme softmax outputs \cite{mishra2025beyond}. However, in the distillation setting the teacher itself is not trained with Mixup, which raises the question of whether the calibration properties of the teacher remain stable when evaluated on interpolated inputs.


\subsection{Information Content of Teacher Predictions}

A key motivation for knowledge distillation is that the teacher logits contain rich information about inter-class relationships. These soft predictions encode similarities between classes that are not captured by one-hot labels.

However, regularization techniques that smooth the output distribution can reduce the amount of information contained in the logits. For example, label smoothing has been shown to erase relational information between classes, which negatively impacts distillation performance \cite{muller2019does}. 

This phenomenon can be interpreted by analyzing the variance of the teacher logits. Let $z_t(x)$ denote the teacher logits. The information content of the prediction distribution can be approximated by the variance across class logits

\begin{equation}
Var(z_t(x)) =
\frac{1}{K}
\sum_{k=1}^{K}
\left(
z_{t,k}(x) - \bar{z}_t(x)
\right)^2
\end{equation}

where $\bar{z}_t(x)$ is the mean logit value.

If interpolated inputs lead to smoother or more uniform predictions, the variance of the logits may decrease, indicating a loss of class-discriminative information available for distillation.


\subsection{Implications for Distillation}

Combining the previous observations, querying a teacher network on Mixup samples introduces two competing effects:

\begin{enumerate}

\item \textbf{Regularization effect.}  
Mixup encourages smoother decision boundaries and may reduce overconfident predictions, potentially improving calibration.

\item \textbf{Information attenuation.}  
Interpolated inputs may reduce the variance of teacher logits, limiting the amount of relational information transferred during distillation.

\end{enumerate}

These effects suggest that the temperature parameter $T$ in the distillation loss plays a critical role. Temperature scaling controls the entropy of the teacher distribution and can compensate for overly sharp or overly smooth predictions.

In particular, increasing the temperature produces a softer distribution

\begin{equation}
p_t^T(x)_i =
\frac{\exp(z_{t,i}(x)/T)}
{\sum_{j=1}^{K}\exp(z_{t,j}(x)/T)}
\end{equation}

which may help restore informative gradients for the student network when the teacher predictions become overly confident or overly smooth.


\subsection{Research Questions}

Based on the previous analysis, we investigate the following questions:

\begin{itemize}

\item How does Mixup affect the entropy and calibration of teacher predictions?

\item Does querying the teacher on interpolated inputs degrade the information content of the logits?

\item Can temperature scaling compensate for the distribution mismatch introduced by Mixup?

\end{itemize}

The following sections empirically evaluate these questions using multiple teacher architectures and student models across CIFAR and ImageNet benchmarks.
